Towards Connecting Control to Perception: High-Performance Whole-Body Collision Avoidance Using Control-Compatible Obstacles

One of the most important aspects of autonomous systems is safety. This includes ensuring safe human-robot and safe robot-environment interaction when autonomously performing complex tasks or in collaborative scenarios. Although several methods have been introduced to tackle this, most are unsuitable for real-time applications and require carefully hand-crafted obstacle descriptions. In this work, we propose a method combining high-frequency and real-time self and environment collision avoidance of a robotic manipulator with low-frequency, multimodal, and high-resolution environmental perceptions accumulated in a digital twin system. Our method is based on geometric primitives, so-called primitive skeletons. These, in turn, are information-compressed and real-time compatible digital representations of the robot's body and environment, automatically generated from ultra-realistic virtual replicas of the real world provided by the digital twin. Our approach is a key enabler for closing the loop between environment perception and robot control by providing the millisecond real-time control stage with a current and accurate world description, empowering it to react to environmental changes. We evaluate our whole-body collision avoidance on a 9-DOFs robot system through five experiments, demonstrating the functionality and efficiency of our framework.

==> ContributionTable.tex <==
While the primitives describing the robot are updated every iteration depending on the robot posture $\mathbf{q}$, those for the environmental obstacles are given by the digital twin before each motion. The embedment of our retrofittable collision avoidance control into the robot control loop, the primitive description, and the algorithm itself are presented in the next subsections. Therein, inter alia, the smooth force calculation, the damping design for the generated spring-mass-damper system and the control of the robot with a mobile base are discussed. All the mentioned points in this paragraph are part of our contribution, listed in Tab. \ref{tab:Contribution}.
\begin{table}[tpb]
    \centering
    \caption{Comparison with other collision avoidances}
    \vspace{-0.2cm}
    \begin{tabular}{l|ccccc}
        \toprule
        Feature & \cite{Dietrich2011} & \cite{Lei2020} & \cite{Jang2021a} & \cite{Scimmi2021} & Ours  \\ 
        \midrule
        Full-body \SI{}{\milli \second} real-time control   &\checkmark&          &          &          &\checkmark\\
        Smooth control                                      &\checkmark&\checkmark&\checkmark&          &\checkmark\\
        Efficient coll. models with all shapes              &          &          &          &          &\checkmark\\
        Full self-collision avoidance                       &\checkmark&          &\checkmark&          &\checkmark\\
        Full-body object collision avoidance                &\checkmark&          &\checkmark&\checkmark&\checkmark\\
        Energy dissipation                                  &\checkmark&          &          &          &\checkmark\\
        Joint limit avoidance                               &\checkmark&          &          &          &\checkmark\\
        Evasive mobile base motions                         &          &          &\checkmark&          &\checkmark\\
        Task \& velocity adaptive                           &          &          &          &          &\checkmark\\
        Easy collision object placement                     &          &          &          &          &\checkmark\\
        Digital twin system integration                     &          &          &          &          &\checkmark\\
        \bottomrule
    \end{tabular}
    \label{tab:Contribution}
    \vspace{-0.3cm}
\end{table}

==> FigGraspedObj.tex <==
\begin{figure}[tpb]
    \centering
    \begin{subfigure}{0.49\columnwidth}
        \input{graphics/GraspedObj_img.pdf_tex}
        \subcaption{Tool and grasped object}
        \label{subfig:GraspedObj:img}
    \end{subfigure}
    \begin{subfigure}{0.49\columnwidth}
        \input{graphics/GraspedObj_plot.pdf_tex}
        \subcaption{Primitive description of (a)}
        \label{subfig:GraspedObj:plot}
    \end{subfigure}
    \vspace{-0.1cm}
    \caption{(a) shows the robot grasping an object with its tool and (b) shows its primitive representation, including tool and grasped object.}
    \label{fig:GraspedObj}
    \vspace{-0.8cm}
\end{figure}
